How does Simulation-based Testing for Self-driving Cars match Human Perception?

Software metrics such as coverage and mutation scores have been extensively explored for the automated quality assessment of test suites. While traditional tools rely on such quantifiable software metrics, the field of self-driving cars (SDCs) has primarily focused on simulation-based test case generation using quality metrics such as the out-of-bound (OOB) parameter to determine if a test case fails or passes. However, it remains unclear to what extent this quality metric aligns with the human perception of the safety and realism of SDCs, which are critical aspects in assessing SDC behavior. To address this gap, we conducted an empirical study involving 50 participants to investigate the factors that determine how humans perceive SDC test cases as safe, unsafe, realistic, or unrealistic. To this aim, we developed a framework leveraging virtual reality (VR) technologies, called SDC-Alabaster, to immerse the study participants into the virtual environment of SDC simulators. Our findings indicate that the human assessment of the safety and realism of failing and passing test cases can vary based on different factors, such as the test's complexity and the possibility of interacting with the SDC. Especially for the assessment of realism, the participants' age as a confounding factor leads to a different perception. This study highlights the need for more research on SDC simulation testing quality metrics and the importance of human perception in evaluating SDC behavior.

==> imgs/tikz/C3S2.tex <==

\resizebox{!}{2cm}{
\begin{tikzpicture}
\draw[gray, thick] (18.991225107372394,10.000000000000002) -- (18.79579513623748,12.60422777072825);
\end{tikzpicture}
}

==> imgs/tikz/C4S1.tex <==

\resizebox{!}{2cm}{
\begin{tikzpicture}
\draw[gray, thick] (18.991225107372394,10.000000000000002) -- (18.79579513623748,12.60422777072825);
\end{tikzpicture}
}

==> imgs/tikz/C4S2.tex <==

\resizebox{!}{2cm}{
\begin{tikzpicture}
\draw[gray, thick] (18.991225107372394,10.000000000000002) -- (18.79579513623748,12.60422777072825);
\end{tikzpicture}
}

==> sections/08-acknowledgement.tex <==
%\section*{Acknowledgement}
We thank the Horizon 2020 (EU Commission) support for the project COSMOS (DevOps for Complex Cyber-physical Systems), Project No. 957254-COSMOS).



==> sections/10-credit.tex <==
\section{CRediT authorship contribution statement}
\textbf{Christian Birchler}: Conceptualization, Data Curation, Formal Analysis, Investigation, Methodology, Project Administration, Resources, Software, Validation, Visualization, Writing – Original Draft Preparation.
\textbf{Tanzil Kombarabettu Mohammed}: Conceptualization, Data Curation, Formal Analysis, Investigation, Methodology, Project Administration, Resources, Software, Visualization.
\textbf{Pooja Rani}: Methodology, Supervision, Writing – Review \& Editing.
\textbf{Teodora Nechita}: Data Curation, Methodology.
\textbf{Timo Kehrer}: Methodology, Resources, Supervision, Writing – Review \& Editing.
\textbf{Sebastiano Panichella}:Conceptualization, Funding Acquisition, Methodology, Project Administration, Resources, Supervision, Writing – Review \& Editing.



%CRediT Classification:
%Conceptualization
%Ideas; formulation or evolution of overarching research goals and aims.
%
%Data Curation
%Management activities to annotate (produce metadata), scrub data and maintain research data (including software code, where it is necessary for interpreting the data itself) for initial use and later reuse.
%
%Formal Analysis
%Application of statistical, mathematical, computational, or other formal techniques to analyze or synthesize study data.
%
%Funding Acquisition
%Acquisition of the financial support for the project leading to this publication.
%
%Investigation
%Conducting a research and investigation process, specifically performing the experiments, or data/evidence collection.
%
%Methodology
%Development or design of methodology; creation of models.
%
%Project Administration
%Management and coordination responsibility for the research activity planning and execution.
%
%Resources
%Provision of study materials, reagents, materials, patients, laboratory samples, animals, instrumentation, computing resources, or other analysis tools.
%
%Software
%Programming, software development; designing computer programs; implementation of the computer code and supporting algorithms; testing of existing code components.
%
%Supervision
%Oversight and leadership responsibility for the research activity planning and execution, including mentorship external to the core team.
%
%Validation
%Verification, whether as a part of the activity or separate, of the overall replication/reproducibility of results/experiments and other research outputs.
%
%Visualization
%Preparation, creation and/or presentation of the published work, specifically visualization/data presentation.
%
%Writing – Original Draft Preparation
%Creation and/or presentation of the published work, specifically writing the initial draft (including substantive translation).
%
%Writing – Review & Editing
%Preparation, creation and/or presentation of the published work by those from the original research group, specifically critical review, commentary or revision – including pre- or post-publication stages.
%
%
%An example of an Authors’ Contribution statement using CRediT with degree of contribution:
%
%Pierro Asara: review and editing (equal). Kerys Jones: Conceptualization (lead); writing – original draft (lead); formal analysis (lead); writing – review and editing (equal). Elisha Roberto: Software (lead); writing – review and editing (equal). Hebei Wang: Methodology (lead); writing – review and editing (equal). Jinnie Wu: Conceptualization (supporting); Writing – original draft (supporting); Writing – review and editing (equal).


==> sections/old/02-old-study-design.tex <==
\section{Study design}\label{sec:study-design}

\begin{figure*}[t]
    \centering
            \vspace{-4mm}
    \includegraphics[width=0.89\textwidth]{imgs/study-overview}
        \vspace{-8mm}
    \caption{High-level overview of the empirical study}
    \label{fig:study-overview}
    \vspace{-4mm}
\end{figure*}


%Pooja focuses on RQ\\
%\todo{we repeat goal and questions}
%\todo{
%Aims:
%\begin{itemize}
%    \item To investigate the perceived level of safety and realism in simulation-based SDC test cases.
%    \item To explore the factors that make simulation-based SDC test cases safe and realistic.
%    \item To investigate the differences in safety and realism when tested in \beamng and \carla.
%\end{itemize}
%Objectives:
%\begin{itemize}
%    \item To immerse average humans in VR to assess the safety and realism test cases
%    \item To survey the experiment participants
%    \item To perform statistical tests on experiment and survey data
%\end{itemize}
%}


% \todo{GENERAL NOTE: Reference ICSE papers to write ours: The Impact of Test Case Summaries on Bug Fixing Performance: An Empirical Investigation, ICSE, 2016. Why Don't Developers Detect Improper Input Validation?': DROP TABLE Papers - https://dl.acm.org/doi/10.1109/ICSE43902.2021.00054}

Overall, our research aims to investigate the extent to which quality metrics (i.e., OOB in our study) of simulation-based test cases of SDCs match human perception and and understand the rationale behind it.
Specifically, we focus on investigating the factors that make simulation-based SDC test cases as safe, unsafe, realistic, or unrealistic. 
Hence, with \framework (framework detailed in Section \ref{sec:approach}), we conducted an empirical study involving 50 participants (recruiting  explained in Section \ref{sec:survey}), with several steps (summarized by Figure \ref{fig:study-overview}) devised to collect different types of evidence and data to answer our main question.  
For this purpose, the usage of \framework allowed the participants involved in our study to immerse themself in virtual SDCs within widely used virtual environments, thanks to virtual reality (VR) technologies (as detailed in Section \ref{sec:approach}, Section \ref{sec:test-generation}, Section \ref{sec:survey}, and Section \ref{sec:experimental-procedure}). 

We structured our study around three main research questions (RQs), in which the participants were asked to assess the level of safety and realism of multiple simulation-based test cases for SDCs.
The first research question investigates the extent to which OOB safety metric for simulation-based test cases of SDCs aligns with the safety assessments of our participants.
\begin{tcolorbox}
%\RQ{1}: To what extent do safety metrics for simulation-based test cases of SDCs align with human safety assessments?
\RQ{1}: To what extent does the OOB safety metric for simulation-based test cases of SDCs align with human safety assessments?
\end{tcolorbox}
%\begin{itemize}
    %\item We conjecture that safety metrics (in general) used in SE do not align with the human perception of safety.
    %\item What is the OOB metric? Why did we select it?
 %   \item What is human perception?
  %  \item What does alignment mean?
   % \item How do we assess the (mis) alignment between human perception and the OBB metric? 
%\end{itemize}

%\RQ{1} addresses the main goal of the study, which is to find out how participants view SDC test failures and their level of safety, with and without virtual reality (VR) technologies. Here, we conjecture that safety metrics (in general) used in software engineering, in our study the OBB metric, do not always align with the human perception of safety. It is important to note that, the alignment (or misalignment) is measured (as described in the following sections, using Likert-scale responses from the participants and correlating/associating it with the occurrence of failing and non-failing test cases.
%Moreover, we conducted statistical tests on experiment and survey data to understand whether the usage of specific simulators (\beamng v.s. \carla), or driving views (i.e., the outside view and the driver’s view, as detailed in the following sections and visualized in Figure \ref{fig:study-overview}) as well as the complexity of test cases (e.g., with and without obstacles and vehicles) impact the safety perception of SDC-generated test cases by the participants.
%After participants expressed their assessment of the level of safety of SDC test cases (\RQ{3}), we asked them to evaluate the extent to which failing and passing SDC test cases are realistic from their point of view. Therefore, our second research question is:
%\begin{tcolorbox}
%%\RQ{2}: How do humans assess the level of realism of failing and passing simulation-based SDC test cases?
%%\cb{The following RQ needs to be redefined.}
%%\RQ{2}: How realistic are failing and passing test cases from a human point of view?
%\RQ{2}: How realistic are test cases from a human point of view?
%\end{tcolorbox}
%\pr{
%\begin{itemize}
%\item From the first RQ, we know that OOB metric match sufficiently matches the human perception of the safety of test cases. However, some safe/unsafe test cases be realistic or unrealistic from the perception of humans.  
%\item Understanding the factors contributing to the test cases' realism can help developers design more realistic test cases.
%\item We used an identical setting of experiments as for \RQ{1}, to answer this question. We design a semi-structured interview followed by a survey to answer this question. In this scenario, we do not consider the interaction between the individual and the car to capture the perception solely.
%\end{itemize}
%}
In \RQ{1} we investigate the extent to which the OOB metric matches the human perception of the safety of SDC test cases. However, some failing and non-failing test cases can be perceived (using Likert-scale responses) as 
%realistic or 
unrealistic by participants.  
Understanding the factors contributing to the test cases' realism can help SDC developers design more realistic test cases in future research.
We applied the same experimental setting to answer \RQ{2} (i.e., a survey with experiments involving our participants, etc.) as \RQ{1}.
Once explored \RQ{1} (perceived level of safety of SDC test cases) and \RQ{2} (perceived level of realism of SDC test cases), we  investigate the impact of the \textit{human-based interactions with the virtual SDCs} (meaning the ability to slow or fasten the SDC behavior during a test case) in assessing the safety and realism of the test cases. 
When individuals can proactively interact with the SDC, it is unclear whether they perceive the test cases as safer/unsafer or more/less realistic.
Therefore, our last research question is:
\begin{tcolorbox}
\RQ{2}: To what extent does the assessment of safety of simulation-based SDC test cases vary when humans can interact with the SDC?
% Alternatives:
%How do human perceptions of safety and realism of simulation-based self-driving car test cases change when humans are able to interact with the self-driving car?
%To what extent do the results of simulation-based testing align with human evaluations of safety and realism in self-driving car test cases when human interaction is involved?
\end{tcolorbox}
To measure the impact of such interaction on the perception of safety and realism of SDC test cases, we provided our participants with the ability to influence the behavior of the SDC when desired (as detailed in the next sections). Then, we analyzed our survey data to derive the most important lessons learned for \RQ{3}. 
%\pr{what do we mean by assessment? Is it human assessment or automatic assessment? Is it from RQ2?}

%In this scenario, we do not consider the interaction between the individual and the car to capture the perception solely.

%\pr{We only measure realism in this question, not safety. The next question focuses on and builds upon both aspects, safety, and realism.}
%\pr{a table with level of realism, techniques to pass and fail test cases}
\RQ{1} addresses the main goal of the study, which is to find out how participants view SDC test failures and their level of safety, with and without virtual reality (VR) technologies. Here, we conjecture that safety metrics (in general) used in software engineering, in our study the OBB metric, do not always align with the human perception of safety. It is important to note that, the alignment (or misalignment) is measured (as described in the following sections, using Likert-scale responses from the participants and correlating/associating it with the occurrence of failing and non-failing test cases.
Moreover, we conducted statistical tests on experiment and survey data to understand whether the usage of specific simulators (\beamng v.s. \carla), or driving views (i.e., the outside view and the driver’s view, as detailed in the following sections and visualized in Figure \ref{fig:study-overview}) as well as the complexity of test cases (e.g., with and without obstacles and vehicles) impact the safety perception of SDC-generated test cases by the participants.
After participants expressed their assessment of the level of safety of SDC test cases (\RQ{3}), we asked them to evaluate the extent to which failing and passing SDC test cases are realistic from their point of view. Therefore, our second research question is:
\begin{tcolorbox}
%\RQ{2}: How do humans assess the level of realism of failing and passing simulation-based SDC test cases?
%\cb{The following RQ needs to be redefined.}
%\RQ{2}: How realistic are failing and passing test cases from a human point of view?
%\RQ{3}: How realistic are test cases from a human point of view?
\RQ{3}: How realistic are test cases considered from a human point of view?
\end{tcolorbox}

\subsection{Experimental Setting}\label{sec:sudy-context}
Our experiments were conducted in a constant and consistent setting.
We elaborate on the following aspects:
\begin{inparaenum}[(i)]
    \item the study design,
    \item the \framework framework,
    \item the used test cases, and
    \item the survey design.
\end{inparaenum}

\subsubsection{Study Design Overview}
Figure~\ref{fig:study-overview} depicts our four-level steps research methodology designed to answer our RQs:
%We describe the research methodology from experiment setup to survey and log analysis.

%\christian{@all: What do you think of having the following sections named as the five steps/phases mentioned below? I guess this would give a more logical flow of this chapter for the reader.}

        %\begin{enumerate}   \item 
            \textbf{(1) Experiment Setup \& Recruiting}: First, we set up the experiment by planning the overall process and generating a dataset of SDC test cases with \framework. We conducted a pilot experiment with a virtual reality expert/researcher (pilot study), thereby enhancing the experimental setup before proceeding with the actual experiments. 
            After finalizing the setup of the experiments, we recruited study participants. We used various recruiting methods (as explained in Section \ref{sec:survey}). We recruited 
            %\seba{next number to be updated/checked} 
            \participantscount  for our experiment. 
            %\item 
            
            \textbf{(2) Introduction to
the Study \& Pre-survey}: Once we identified the participants, we briefly described the study, and sent them a pre-survey (the day before the experiment). The pre-survey provided a high-level introduction to our experiment and a disclaimer clarifying that we will proceed with anonymizing data considering that virtual environment accidents can be experienced during the experiments. In this phase we also collected participants' background information: demographic, work/driving experience, and VR experience data.
            %\item 
            
            \textbf{(3) Experiments}: 
       In the experimentation phase, asked the participants to take part in various experiments and collected feedback. During this phase, we shared with the participants a survey, to guide them during the required steps of the experiments.
            %\item 
            
            \textbf{(4) Analysis of Experimental Data}:
            We analyzed the survey and participant logs, to answer questions \RQ{1}, \RQ{2}, and \RQ{3}. \\
         
    %\end{enumerate}
        The following sections elaborate on the approach proposed to answer our RQs and detail the methodological steps, including the survey design and experimental procedure.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{imgs/sdc-alabaster-architecture.png} % https://drive.google.com/file/d/1YWj_Kp0w7kKSPHirNs6D-IC7hIctZ5aq/view?usp=sharing
                %\vspace{-5mm}
    \caption{\framework Architecture Overview \seba{@Chris, make the font size of text bigger (if necessary make it bigger the component elements (keep the image to a single column, to save space))}}
    \label{fig:sdc-alabaster-architecture-overview}
                %\vspace{-2mm}
\end{figure}

\subsubsection{\framework approach}
\label{sec:approach}
%\todo{Overview our \framework framework.}
%\pr{SDC-Alabaster workflow in very brief, Maybe (fig 3.1, fig 3.3 in the replication package) fig 3.7}

%\framework allows humans to assess the level of safety and realism of multiple simulation-based test cases for SDCs (based on virtual environments such as \beamng and \carla) by leveraging virtual reality (VR) technologies~\cite{9889526}.
The architecture overview of \framework can be visualized in Figure~\ref{fig:sdc-alabaster-architecture-overview}, which provides a general view of all its components (Table~\ref{tab:components-input-output} reports the essential inputs and outputs of the main components) and how they interact with each other to enable the \framework' automation.

It is important to highlight that \framework is built on top of \sdcscissor (a reference technology for generating and selecting SDC test cases \cite{DBLP:journals/ese/BirchlerKBGP23,DBLP:journals/tosem/BirchlerKDPP23,DBLP:conf/wcre/BirchlerGKGP22,BIRCHLER2023102926}) and VR technologies~\cite{9889526}, and implements additional components (see Figure~\ref{fig:sdc-alabaster-architecture-overview}), to enable humans to immerse themself in a virtual SDC.
%We built \framework on top of 
\sdcscissor was selected as the main open source technology since it provides an easy-to-use infrastructure for running customized simulation-based test cases for SDCs, and it abstracts low-level aspects of the simulation environment away, such as the interpolating and spawning of the environment.
Test cases in such an environment are classified as failing and passing test cases based on the OOB metric.
Due to the modular, open-source architecture of \sdcscissor we were able to extend the tool with additional components integrating VR technologies.
%\seba{@Christian, in the following line, for both Dreye VR and vorpX we should have sentences, maybe between parenthesis, describing what such tools do/are. Consider the SDC-scissor sentence "(a reference technology for generating and selecting SDC test cases \cite{DBLP:journals/ese/BirchlerKBGP23,DBLP:journals/tosem/BirchlerKDPP23,DBLP:conf/wcre/BirchlerGKGP22,BIRCHLER2023102926})". We need a similar sentence for each tool in the following paragraph}.
Specifically, \framework integrates \dreye (i.e., \carla with VR feature) from~\cite{DBLP:conf/hri/SilveraBA22} and \vorpx~\cite{vorpx} (i.e., driver for converting graphics output to a compatible format for VR), which allows us to visualize \carla and \beamng into VR headsets, so that humans can immerse themself into the virtual environments and  assess SDCs's behavior. 
%\seba{@Christian, shell we mentioned that \framework builds upon \textsc{DReye VR} from~\cite{9889526}, or we mainly refer to it in the related work? I would prefer only to mention shortly in related work. What do you think?}
Hence, from a technological standpoint, as shown in Figure~\ref{fig:sdc-alabaster-architecture-overview}, it is possible to observe that \framework leverages external components (e.g., simulators and VR-related hardware) as well as internal/new components we developed.
%: the Human Component Interactor, the HCI Interpreter, and the HCI Actuator. 
We detail such components in the next paragraphs.


%\paragraph{External Components} 
\textbf{External Components.} 
\framework relies also on external components, which were developed by third parties and recent research. They are represented as orange and violet components in Figure~\ref{fig:sdc-alabaster-architecture-overview}.
Concretely, \framework requires simulators, such as \beamng and \carla as well as VR-related hardware to immerse the users into the simulator.
%
%\paragraph{Simulators}
As indicated in Figure~\ref{fig:sdc-alabaster-architecture-overview}, \framework uses two simulators (orange components), namely \beamng, and \carla since they implement fundamentally different physics behavior.
We use \beamng since this simulator is a well-known reference technology used in recent years in several publications and software engineering events on SDC testing~\cite{BeamNGresearch,9476243,SBST2022,DBLP:journals/ese/BirchlerKBGP23,DBLP:journals/tosem/BirchlerKDPP23,DBLP:conf/wcre/BirchlerGKGP22,BIRCHLER2023102926}.
The \beamng simulator comes along with a soft-body physics engine that allows the simulation of body deformations and therefore more realistic simulations regarding crashes and impacting foces on objects.
On the other hand, \beamng does not allow headless simulations which means that all simulations must be rendered~\cite{DBLP:journals/ese/BirchlerKBGP23,DBLP:journals/tosem/BirchlerKDPP23,DBLP:conf/wcre/BirchlerGKGP22,BIRCHLER2023102926}.
\beamng provides a Python API called \textit{beamngpy}~\cite{BeamNGpy} so that \framework can interact with the simulator and send the actions.
Complementary, another widely used simulator in industry and academia is \carla~\cite{DosovitskiyRCLK17, 10.1007/978-3-030-60508-7_9, DBLP:conf/aaai/NairSAK21, DBLP:journals/mta/HuelamoEBBGAAL22, DBLP:conf/infocom/ZhangFCJZX20, DBLP:journals/sensors/Gutierrez-Moreno22}.
%\seba{@christian, in the next sentences try to describe what are the differences between rigid-body physics engines (now it is not clear), which works differently than soft-body physics. Do the same for the test specifications of the simulators. In doing so, consider that we do not have too much space. Limit yourself in 1-2 sentences for each of the aspects I refer to above}
The differences between \carla and \beamng are twofold.
On one hand, \carla comes with a rigid-body physics engine, which works differently than the soft-body physics engine of \beamng.
A rigid-body simulation environment does not deform objects, e.g., when a crash happens.
On the other hand, the test specifications of these simulators are different.
\beamng requires coordinate points (i.e., sequences of X and Y-coordinates) in order to define a test track whereas \carla relies on the \textit{ASAM OpenDRIVE} format~\cite{opendrive-format}.
Despite those differences, \carla also provides a Python API~\cite{carlapy} to manage the simulations, which allowed a stable integration into \framework.
%\seba{@christian, add a line here, stating that for the first time, both these two simulators have been used for generating failing and passing scenarios, as well as for assessing SDC test cases from a human point of view. This is critical and should be mentioned concisely among the contributions of the work in the introduction.}
%
%\paragraph{Virtual Reality Hardware}
Another external component covers the area of Virtual Reality (VR), as visualized in Figure~\ref{fig:sdc-alabaster-architecture-overview} and Figure~\ref{fig:workflow}.
This component is the main software leveraging the VR hardware such as VR headsets to immerse users into the simulation environment.
We argue, the more the users feel to be in a real environment the more acurate are the assessment of the test cases.
Concretely, by using VR headsets we enable the user to experience a 360° view so that the assesment of the test cases are not constrained to the limited view that a normal monitor provides.
We implemented \framework so that it works with two VR headsets namely
\begin{inparaenum}[(i)]
    \item \vive, and
    \item \oculus.
\end{inparaenum}
%The VR headset \vive (Figure~\ref{fig:sdc-alabaster-architecture-overview}) immerses the user in a virtual environment.
The \vive headset has no onboard GPU for simulation but a wired connection to an external device with a dedicated GPU.
In contrast to \vive, the \oculus headset is able to operate wired and wireless.
For the wireless operation of the device, \oculus has an onboard GPU for rendering.
%However, we suggest using a wired connection to an external, more powerful GPU for better simulation performances.
%Both VR technologies come with different features, which enable \framework to be used in different use cases.
%Depending on the user's needs, the appropriate VR technology can be selected.
An overview of the features provided by \vive and \oculus is shown in Table~\ref{tab:vr-feature-overview}.
%\seba{the above part still does not clarify what aspects/characteristics of such VR headsets are important for running our study, how our software interact with them, etc., @christian, can we elaborate more on it (maybe also shortening/commenting out what is not necessary?)?}

\begin{table}[t]
    \centering
    \caption{Features of \vive and \oculus 
    %\seba{not fully clear all numbers units in the table, please quality with units what we are referring to..}
    }
    \small
    \begin{tabularx}{\linewidth}{ccc}\toprule
         \textbf{Feature}       & \textbf{\vive} & \textbf{\oculus} \\ \midrule
         Onboard GPU            & \xmark    & \cmark \\ 
         Wired connection       & \cmark    & \cmark \\ 
         Wireless connection    & \xmark    & \cmark \\ 
         Peripherals            & \cmark    & \cmark \\ 
         Android OS             & \xmark    & \cmark \\ 
         Windows OS             & \cmark    & \xmark \\ \bottomrule
    \end{tabularx}
    \label{tab:vr-feature-overview}
\end{table}

%\paragraph{Internal Components}
\textbf{Internal Components.}
\framework builds upon \sdcscissor \cite{DBLP:journals/ese/BirchlerKBGP23,DBLP:journals/tosem/BirchlerKDPP23,DBLP:conf/wcre/BirchlerGKGP22,BIRCHLER2023102926} by extending it with additional new, independent components (Figure~\ref{fig:sdc-alabaster-architecture-overview}).
This makes \framework the first framework combining virtual reality technologies with regression testing techniques  for SDC software (i.e., \sdcscissor \cite{DBLP:journals/ese/BirchlerKBGP23,DBLP:journals/tosem/BirchlerKDPP23,DBLP:conf/wcre/BirchlerGKGP22,BIRCHLER2023102926}).
Specifically, \framework implements components that interact with each other over its APIs:
\begin{inparaenum}[(i)]
   \item a Human Component Interactor (HCI),
   \item an HCI Interpreter, and
   \item an HCI Actuator.
\end{inparaenum}

%\paragraph{Human Component Interactor (HCI)}
\seba{@Christian, the following part is not clear, please improve it. Consider that we need to have a sentence saying what this component goal/task is, why it is important, and  how human inputs are collected by it (when, why, and what format is used, etc.). Consider updating Table \ref{tab:components-input-output} accordingly. When possible, explain also how the VR headsets,  \dreye,  \vorpx, and the simulators (\carla and \beamng) interact with each other and with \sdcscissor. At the moment, all such aspects are too high-level (see part below on external component, to see the level of detail we use there). } 
This component is the main component the user interacts with.
It takes as input any user interaction from the keyboard and forwards it toward the HCI Interpreter component.
The next component, the HCI Interpreter, will further process the interaction.


%\paragraph{HCI Interpreter}
\seba{@Christian, the following part is not clear, please improve it. Consider that we need to have a sentence saying what this component goal/task is, why it is important, and  how human inputs are collected/analyzed by it (when, why, and what format is used, etc.). Consider updating Table \ref{tab:components-input-output} accordingly. When possible, explain also how the VR headsets,  \dreye,  \vorpx, and the simulators (\carla and \beamng) interact with each other and with \sdcscissor. At the moment, all such aspects are too high-level (see part below on external component, to see the level of detail we use there). } 
\seba{@Christian, what interactions we are talking about in the next sentence? I believe that this should be explained in the previous component (Human Component Interactor), so that here we refer only on how we store/analyze/interpret the information}
The forwarded interaction from the HCI component is interpreted by the HCI Interpreter and produces a generic command for the simulators.
The HCI Interpreter only allows certain pre-defined interactions for the user.
%We have to mention that due to technical limitations such as the fact that an AI is driving the car a user can not specify the vehicle's speed manually; for instance, the user is only allowed to set the vehicle's maximum speed with specific keystrokes on the keyboard.
Then, the component analyzes the type of interaction and its values so that it can generate a generic command for the simulators.


%\paragraph{HCI Actuator}
\seba{@Christian, the following part is not clear, please improve it. Consider that we need to have a sentence saying what this component goal/task is, why it is important, and  how human inputs are collected/analyzed by it (when, why, and what format is used, etc.). Consider to update Table \ref{tab:components-input-output} accordingly. When possible, explain also how the VR headsets,  \dreye,  \vorpx, and the simulators (\carla and \beamng) interact with each other and with \sdcscissor. At the moment, all such aspects are too high-level (see part below on external component, to see the level of detail we use there). } 
\seba{@Christian, what commands we are talking about in the next sentences? I believe that this should be explained in the previous component (HCI Interpreter), so that here we refer only on how we store/analyze/use the information}
The HCI Actuator gets as input a generic command for the simulators.
This component processes the generic abstract command and produces specific commands for each simulator (i.e., \beamng and \carla) since the API for the simulators are different and therefore require different implementations.
The concrete simulators will be invoked with the generated commands from this component.

\begin{table}[t]
    \centering
    \scriptsize
    \caption{Overview of components' input and output. \seba{@Christian, this table is too generic, make it more accurate detailed in the actual used inputs and output (e.g., adding a column on the format of the input, and enhancing the descriptions.) } }
                \vspace{-3mm}
    \begin{tabularx}{\linewidth}{llX}\toprule
         \textbf{Component} & \textbf{Input}    & \textbf{Output}  \\ \midrule
         HCI                & User interactions             & Input representation  \\
         HCI Interpreter    & Input representation          & Generic command representation for simulators  \\
         HCI Actuator       & Generic command               & Specific command for \beamng or \carla \\
         Simulators         & Specific simulator command    & Video output \\
         Virtual Reality    & Video output                  & Immersive video output for VR headsets \\ \bottomrule
    \end{tabularx}
    \label{tab:components-input-output}
                \vspace{-3mm}
\end{table}

%\paragraph{Log interactions} %\seba{@Christian, add here details on log interaction reported visually in Figure \ref{fig:sdc-alabaster-architecture-overview}... }
All interactions with the simulation environment (i.e., keystrokes to ajdust the maximum speed) are logged and preserved.
Based on those logs, we can evaluate to what extent the user interacted with the SDC.

%\paragraph{Infrastructure requirements} % \seba{@Christian, add here details on the GPU minimal requirements and expectations to make the full automation of \framework operate. Not sure I would create a table. I would mainly list the main requirements as text (indeed commented the table in the latex)}
\textbf{Infrastructure requirements.}
To run \framework, several hardware and software requiremnts are required such as
\begin{inparaenum}[(i)]
    \item VR headset,
    \item performant GPU,
    \item right operating system,
    \item installation of simulators, and
    \item the \framework framework.
\end{inparaenum}

For our experiments (see Section~\ref{sec:experimental-procedure}), we use \vive as our VR technology.
This device is allows us to immerse the user with a high resolution of the virtual environment compared to other VR technology such as the \oculus.
The \vive, however, requires a dedicated external GPU device.
In our setting we use the \textit{nVidia GeForce RTX 3080}, which is compatible with \vive, together with \textit{Windows 10} as our operating system.

Furthermore, the installation of \beamng and \carla require additional extensions.
Since \beamng does not provide a built-in support for VR, we need to install \vorpx, which is a general purpose VR driver that projects the computer screen on a 2.5D surface.
In the case of \carla, we need to install the \textit{DReyeVR} extension of \cite{DBLP:conf/hri/SilveraBA22}.
This extension allows a full VR experience inside the \carla simulation environment.
If all requirements are met, \framework needs to be installed to run the test cases in the simulaion environemnts and to immerse the user.



\subsubsection{Test case generation with \framework}
\label{sec:test-generation}
Our study consists of (i) objects, i.e., SDC test cases generated by \framework , and (ii) participants assessing the safety and realism of generated test cases. In this section, we describe how we generated SDC test cases with \framework, while in the next one, we discuss how we conducted our survey-based assessment involving humans.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{imgs/road-points.jpeg}
    \vspace{-2mm}
    \caption{Road points as SDC test specification}
    \label{fig:road-points}
    \vspace{-2mm}
\end{figure}

%\paragraph{\framework Workflow}
\textbf{\framework Workflow.}
\cb{I am not sure if we should have the workflow in this section since it should be only about the test generation itself, i.e., about test specification and test generators from SBST.}
The workflow of \framework is illustrated in Figure~\ref{fig:workflow}.
\framework leverages \sdcscissor to apply the same concept for specifying test cases for SDCs: A test is simply specified in a JSON file by a sequence of XY-coordinates, which are referred to as road points.
The actual road in the virtual environments is the result of interpolating the road points as illustrated in Figure~\ref{fig:road-points}.
Creating the test cases manually by testers is not feasible since specifying the sequences of road points can be a cumbersome task.
To overcome this issue, we leverage state-of-the-art test generators for SDCs~\cite{DBLP:conf/sbst/CastellanoCTKZA21, SBST2022, 9476243, 9810738, 9810692} that automatically generate those road points.
The user can then invoke the test generation process of \framework by choosing the top-ranked state-of-the-art test generators for SDCs available come from the tool competition of the Intl. Workshop on Search-Based Software Testing (SBST): Frenetic, FreneticCV, and Ambiengen~\cite{9476243, SBST2022}. 
It is important to note that integrating such generators in \framework, to apply them for both \beamng and \carla simulators, required us to perform specific adaptations/implementations since \carla and \beamng have different APIs.
%\seba{@Chris, I guess we could add the references to the actual test generators in the above sentences)}

\framework persists all generated test cases as JSON files containing the road specifications which will be further processed in the next step for the simulation environments of \beamng or \carla.
Depending on the actual simulator that will be used, \framework translates the road specifications to the simulator-specific environment.
As input, \framework takes the road specifications obtained from the previous phase, and an option specifies which simulator (\beamng or \carla) is used for running the tests.
Then, the user is immersed in the virtual environment with the VR headsets, experiencing SDC test cases.
%\framework automatically generates a variety of test cases for \beamng and \carla  using the test generators.

The following paragraphs provide more details of the implementation of the test generators  into \framework.
Furthermore, we will elaborate on the technical use of VR with the different simulators for immersing the users into virtual environments.

\begin{figure}[t]
    \centering
\includegraphics[width=0.48\textwidth]{imgs/workflow.png} % https://drive.google.com/file/d/1Q2pVa-IfgHEXTC_AnkEeN0n9zos6q4rV/view?usp=sharing
        %\vspace{-5mm}
    \caption{\framework's workflow overview}
    \label{fig:workflow}
        %\vspace{-5mm}
\end{figure}

%\paragraph{Test Generators \& Integration in VR}
\textbf{Test Generators \& Integration in VR.}
The test generators from the tool competition of SBST workshop~\cite{9476243, SBST2022} are developed as an integrated platform leveraging the \beamng simulator. \footnote{\url{https://github.com/se2p/tool-competition-av}}
%\framework's test specification is based on the SBST tool competition platform, there is a straightforward integration of the test generators into our framework.
%More challenging was to enable the immersion of the user into the virtual environment of \beamng with VR technologies and the integration of static and dynamic objects into the virtual environment.
With \framework, the user can modify the test case scenes by adding different types of objects (i.e., static and dynamic).
When using \framework with the \beamng simulator, the user has the option to add trees, speed bumps, and delimiter to the road. %as illustrated in Figure~\ref{fig:beamng-with-static-objects}.
These objects are placed by specifying the parameter in the test configuration. % (see Listing~\ref{lst:yml-config-file}).
%The integration of objects into the virtual environment should give a different perception of the scenario to the user who is immersed in the simulation scenario.
%\begin{figure}[t] %https://drive.google.com/file/d/1ufCBRcEhEAUcuUP6vX9HeoAND98fwlHC/view?usp=sharing
%    \centering
%    \begin{subfigure}{0.45\textwidth}
%        \includegraphics[width=\textwidth]{imgs/approach/vorpx-top-view.png}
%        \caption{Top view with angle $\alpha$}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}{0.45\textwidth}
%        \includegraphics[width=\textwidth]{imgs/approach/vorpx-side-view.png}
%        \caption{Side view with angle $\beta$}
%    \end{subfigure}
%    \caption{View angles in VR with vorpX}
%    \label{fig:vorpx-view-angle}
%\end{figure}
\beamng has not a built-in solution for using the simulator with VR technologies, thus third-party tools are required to bridge the gap.
We used the VR driver \vorpx, a specialized tool to transform any visual output to the screen to a compatible input for VR headsets so that it gives to a certain extent an immersive feeling for the user.
The \vorpx software gives a broader view angle when wearing a VR headset.
The user can move the head and can explore the virtual environment according to its head movement. 
%However, the view is still limited and does not provide a 360° round view for the user.
%\subsection{\carla}\label{sec:test-generation-carla}
%\begin{figure}[t]
%    \centering
%    \frame{\includegraphics[width=\textwidth, frame]{imgs/approach/carla-with-objects.png}}
%    \caption{\carla with static and dynamic objects}
%    \label{fig:carla-with-static-objects}
%\end{figure}

In the case of the \carla simulator, there is no difference in the use of the test generators.
However, test cases generated are processed differently compared to the \beamng simulator since \carla defines the virtual environment slightly differently. An automatically generated test case contains as mentioned before a sequence of XY-coordinates specifying the road points.
The \carla simulator, however, does not need all the road points defined in the test.
Hence, \framework segments the road definition and only uses the start and end points of the segments to declare the beginning and end of the scenario in \carla.
%The integration of additional objects (static and dynamic) into the \carla simulator allows a more comprehensive understanding of the level of safety perception of the user.
%With \carla, the \framework framework can add easily objects to the environment.
%This modification of the environment can even be done at runtime, i.e., during the test execution.
\seba{@Chris, maybe we could shorten the following part to the essential parts of it}
To enable the immersion of the user and manual safety evaluation of the scenario \framework adapts the test specifications for \carla automatically and uses VR headsets to immerse the user into the \carla's virtual environment.
An extra feature of \carla enables the use of VR for its simulations.
\framework utilizes the HARPLab \footnote{\url{https://github.com/HARPLab/DReyeVR}}  extension project for \carla to enable the VR integration.
The HARPLab project contributes to the development of the VR environment.
When launching the \carla application, passing the \texttt{-VR} flag will put the simulator into VR mode. 
VR mode is in its experimental phase, so it can only be used for one Carla map, and integrating VR controllers requires modifying the simulator's core and cannot be done through the client API. \footnote{\url{https://github.com/HARPLab/DReyeVR/blob/main/Docs/SetupVR.md}}
%Details information on setup can be found on the dedicated repository of HARPLab
%\footnote{\url{https://github.com/HARPLab/DReyeVR/blob/main/Docs/SetupVR.md}}.

%\begin{itemize}
%\item Label test case to run execute the test case          with beamng input home ( path of beamng instance) test (path of test case )         rf,oob,maxspeed,interrupt,obstcales,bump,fieldofview,tree dist output execute of test case
%        
%\item Label carla  test case to run execute the            test case with carla input
%                test (path of test case ), port of carla, 
%                res(resoultion),agent(AI Behavior),behavior (aggressive,caution etc)
%                map\_size,number\_of\_vehicles,number\_of\_walkers,dynamic\_weather,  weather\_change\_frequency,map,driver\_view(flag)
%                output execute of test case
%            
%\end{itemize}

%\paragraph{Test Cases Dataset}
\textbf{Test Cases Dataset.}
In the context of  \RQ{1}, \RQ{2}, and \RQ{3}, we build our dataset of test cases using a sampling strategy 
%to select the three test cases for the experiment  to determine whether SDC test cases are safe or unsafe.
\framework generated 1,000 test cases as arrays of X,Y coordinates of road points, and interpolated the road points to construct the road (see Figure \ref{fig:road-points}). 
%We can see an example of a selected test case from \framework{} in Listing \ref{lst:selectedTestCase}. 
We applied stratified random sampling to select three test cases from the dataset of 1,000 test cases, which was used with both the \carla and \beamng simulators.
\seba{@christian, we need some more information don't the test cases that have been selected. We have test cases for the various RQs, we need to know, how many have been then used for each RQs, and what was the profiles of such test cases (obstacles, nr/ of other vehicles, length of the road, etc.), relation with the RQs (i.e., what test cases have been used for each RQ), information on the fact that the test cases fail or not. A table would be useful (e.g., columns are the RQs (first level) and characteristics of the test cases (second level), and in a rows we have the test cases)}
%The test cases generated by  \framework contains roads, whereas in \carla we use a selection of maps. We divided the generated test case into multiple segments and set a car's destination until it reaches the generated test case's final destination point.
%, as manual sampling can result in bias in dataset selection and reduce sample bias. 
%We used stratified random sampling\footnote{\url{https://www.investopedia.com/terms/stratified_random_sampling.asp}}, in which test cases are divided into smaller, non-overlapping groups.
%When sampling, it is possible to organize these groups and then draw samples from each group separately.
%\begin{figure}[h!]
%\centering
%\begin{minipage}{0.9\textwidth}
%\begin{lstlisting}[caption={Selected test case},label={lst:selectedTestCase},language=json,firstnumber=1]
%{
%  "test_id": 0,
%  "test_outcome": "NOT_EXECUTED",
%  "predicted_test_outcome": null,
%  "test_duration": null,
%  "road_points": [
%        [
%          46.46775185638596,
%          75.47341331328971
%        ]...
%    ],
%    interpolated_road_points": [
%        [
%          46.467751856385966,
%          75.47341331328973
%        ]...
%    ],
%    "simulation_data": []
%}
%\end{lstlisting}
%\end{minipage}
%\end{figure}
%\begin{table*}[h!] 
%	      \vspace{-1.5mm}
%        \centering
%        \scriptsize
%        \caption{Test Case}
%        \label{tab:testcase}
%	      \vspace{0mm}
%%\resizebox{0.99\textwidth}{!}{ %0.75
%	\begin{tabular}{p{3cm}p{6cm}p{1.1cm}}
%	%\begin{tabular}{|p{2cm}|p{7cm}|p{2cm}|p{7cm}|p{7cm}}
%		%\fontsize{9}{9}\selectfont 
%		\toprule
%		%
%		\textbf{Attribute} & \textbf{description} & \textbf{Example}  \\
%		%
%		\midrule
 %       \textbf{test\_id} & Identification of the test case & 0 \\
 %       \textbf{test\_outcome} & Results of the test execution & NOT\_EXECUTED \\
 %        \textbf{predicted\_test\_outcome} & prediction of the test execution & null \\
 %        \textbf{test\_duration} & Time taken to execute the test case & null \\
 %        \textbf{road\_points} & Coordinates of road points & [[100,100]] \\
 %        \textbf{interpolated\_road\_points} & Driving Path Road Coordinates  & [[100,100]] \\
 %        \textbf{simulation\_data} & sensor and simulation data after execution & [] \\
%		\bottomrule
%	\end{tabular}
%} %of resizebox 
%	      \vspace{-5.5mm}
%\end{table*}

\subsubsection{Survey design}
\label{sec:survey}
%\pr{Separate questions from Table 4.5 from the thesis according to the RQ1-3.}

To recruit participants we sent email invitations to our contacts from industrial partners as well as to students and researchers from different departments of various universities. 
We generally, targeted dedicated mailing lists from different institutions and organizations (i.e., including non-computer science organizations) and social media (Twitter, Linkedin, etc.). In addition, physical and digital flyers were used to attract more diverse participants. 
This setting allowed us to identify a set of potential participants with diverse backgrounds and varying levels of education. In the end, \participantscount subjects accepted to take part in our experiment.
%as summarised in 
As shown in Table~\ref{tab:participant-overview}, we have data of 50 study participants from which 18 are women and 32 are men.
\todo{Include more details on age, background etc. Consider to include a table.}
\cb{@Seba: How much details should I provide about the participants}
A day before the actual experiment, we sent the participants an email with the details of 
%the location and time for 
the experiments and a pre-survey. 
%There were XX women and XY men in our study.

\subsection{Study participants statistics}

\begin{table*}[h!]
\caption{Professional Experience of Participants (with \textit{High Educ.} refers to Faculty and/or Senior Researcher)}
\label{table:summarizes_participants}
\centering
%\scriptsize
\begin{tabularx}{0.8\linewidth}{Xccccccc}
\toprule
\multirow{2}{*}{\textbf{Field/Profession}}  & \multicolumn{6}{c}{\textbf{Education level}}                                                              & \multirow{2}{*}{\textbf{Total}}  \\
\cline{2-7} \vspace{-2mm} \\
                                                        & \textit{High Educ.*}  & \textit{Postdoc}  &\textit{PhD}   & \textit{Master}  & \textit{Bachelor} & \textit{other}                                      \\ \midrule    
Artificial Intelligence (AI)    & - & - & - & 1  & - & - & 1\\
AI ethics / Political science   & - & - & 1 & -  & - & - & 1 \\    
Biology                         & - & 1 & 2 & -  & - & - & 3 \\ 
Business Administration         & - & - & - & -  & 2 & - & 2\\   
Computer Science                & 2 & 2 & 5 & 22 & 5 & 1 & 37 \\ 
Robotics                        & - & - & - & 1  & - & - & 1 \\    
Mechanical Engineering          & - & - & - & -  & 1 & - & 1 \\    
Industrial Engineering          & - & - & - & 1  & - & - & 1 \\    
Architecture                    & - & - & - & 1  & - & - & 1 \\    
Law                             & - & - & 1 & -  & - & - & 1 \\    
Commercial Clerk                & - & - & - & -  & - & 1 & 1 \\    
\midrule
Total                           & 2 & 3 & 9 & 26 & 8 & 2 & \textbf{\participantscount }\\
\bottomrule
\end{tabularx}
\end{table*}

%        \begin{figure}[h!]
 %               \centering
 %               \includegraphics[width=\textwidth]{imgs/Participants' age distribution.png} 
  %              \caption{ Participants' age distribution}
  %              \label{fig:participants_age_distribution}
  %      \end{figure}

\subsubsection{Pre-survey}
The pre-survey contains a high-level introduction to the topic and an experimental overview (approximate time, location of experiment, and recommendation to wear contact lenses). In addition, we described the type of simulator and VR headsets used for the experiment. The pre-survey also contained a disclaimer regarding confidentiality and anonymity of personal information, as well as a warning to be prepared for fatalities or accidents, that the participants could experience in VR.
%\begin{tcolorbox}
%\textbf{Disclaimer}:
%All the information that you provide will be treated as confidential and will only be
%used for research purposes. We will not disclose your personal information to third parties.
%To simulate a real-world setting, some driving simulations may lead to fatalities or
%accidents. Please consider your readiness for participating to these
%experiments.
%\end{tcolorbox}
%Following the summary information and disclaimer section of the pre-survey, a yes/no question was asked  to agree to the disclaimer (\textbf{Question: }\textit{Would you accept the above terms and continue participating in the study?}) 
After this, the following section of the pre-survey consisted of collecting background information on the participants
%. We have grouped the questions 
(as summarized in the appendix in our replication package \seba{@Chris, we do not have space for reporting also this question. Can you create an appendix with such pre-survey table of questions and include it in the replication package?}). 
%reported in Table~\ref{tab:questions} 
%into two topics: (i) \textit{Background}, (ii) \textit{Experimental Evaluation}. 
The \textit{Background} questions provided us with  information on the participants such as testing experience, driving experience, the usage of VR technologies, and their age and gender.
%, which helped us provide a guide to evaluating results and provided a background for safety and realism in virtual SDCs.


%\begin{table*}[h!] 
%	      \vspace{-1.5mm}
%\centering
%\scriptsize
%\caption{%\fontsize{9}{9}\selectfont
%Pre-survey questions. (MC: Multiple Choice, OA: Open Answer)
%}
%\label{tab:questions}
	%      \vspace{0mm}
%\resizebox{0.99\textwidth}{!}{ %0.75
%	\begin{tabular}%{p{2.8cm}p{0.5cm}p{5.9cm}p{1.1cm}<{\centering}p{1.6cm}<{\centering}}
	%\begin{tabular}{|p{2cm}|p{7cm}|p{2cm}|p{7cm}|p{7cm}}
		%\fontsize{9}{9}\selectfont 
%		\toprule
		%
%		\textbf{Section} & \textbf{ID} & \textbf{Summarized Question} & \textbf{Type} & \textbf{\# Responses} \\
%		%
%		\midrule
%		%
%		\multirow{6}{*}{\textbf{Background }} & Q1.1 & Full Name? & OA & \participantscount \\
%		& Q1.2 & Email? & MC+OA & \participantscount \\
%		& Q1.3 & You are a(Student/Professional/Both Student and Professional)?  & MC+OA & \participantscount \\
%		& Q1.4 & Education (Currently doing / Completed)
%? & MC+OA & \participantscount \\
%		& Q1.5 & Age? & MC & \participantscount  \\
%		& Q1.6 & What is your field of study or profession ? & MC+OA & \participantscount  \\
		%
%		\midrule
%		\multirow{9}{*}{\textbf{Experimental Evaluation}} & Q2.1 & Do you have any  programming experience ? & MC & \participantscount  \\
%		& Q2.2 & Do you have any  programming experience ?  & MC & \participantscount \\
%		& Q2.3 & Do you drive motorbikes, cars etc? 
 %& MC+OA  & \participantscount \\
%		& Q2.4 & What kind of vehicle do you drive ?
 %& MC+OA & \participantscount \\
%		& Q2.5 &How many years of driving experience do you have? & MC+OA  & \participantscount \\
%		& Q2.6 & How would you rate your driving skills? & MC+OA  & \participantscount \\ 
%        & Q2.7 &  Have you ever use virtual reality(VR)  headset (like Oculus Quest,  HTC VIVE,  HoloLens  etc)? & MC+OA  & \participantscount \\ 
 %       & Q2.8 & Have you ever been in a self-driving car? & MC+OA  & \participantscount \\ 
  %      & Q2.9 & Do you play PC/Consoles Games ? & MC+OA & \participantscount \\ 
		%
%		\bottomrule
%	\end{tabular}
%} %of resizebox 
%	      \vspace{-5.5mm}
%\end{table*}

\subsubsection{Survey questionaires}
Table \ref{tab:simulatorbasedsurvey} summarizes the main questions we asked the participants during the experiments to answer our RQs, which include multiple choice (MC), open answer (OA), and Likert scale (LS) based questions. As follows, the main steps of the experiments conducted with our participants:
\begin{itemize}
    \item An introduction to the topic of research and explanation of VR and simulators, followed by an overview of exploration with the help of survey sections, is used to direct the participant throughout each experimental session.
    \item After each testing session, test cases are visualized and evaluated using post-session questions by each participant.
    \item Each experiment concludes with a question for the participants based on the simulator (see Table \ref{tab:simulatorbasedsurvey}).
    \item At the end of all the experiments, we ask each participant to provide comments on the study (see Table \ref{tab:simulatorbasedsurvey}).
\end{itemize}
In the next section, we elaborate on how we analyzed the experimental data to answer the RQs.

\begin{table}[!htb] 
	      %\vspace{-1.5mm}
\centering
\scriptsize
\caption{\cb{Do we need the last column?} \seba{probably not}\fontsize{9}{9}\selectfont Survey questions. (MC: Multiple Choice, OA: Open answer, LS: Likert scale (1-5, where 1 is worst and 5 is best))}
\label{tab:simulatorbasedsurvey}
	      \vspace{-1mm}
%\resizebox{0.99\textwidth}{!}{ %0.75
	\begin{tabular}{p{1.5cm}p{0.5cm}p{3cm}p{0.8cm}<{\centering}p{1cm}<{\centering}}
	%\begin{tabular}{|p{2cm}|p{7cm}|p{2cm}|p{7cm}|p{7cm}}
		%\fontsize{9}{9}\selectfont 
		\toprule
		%
		\textbf{Section} & \textbf{ID} & \textbf{Question(s)} & \textbf{Type} & \textbf{\# Resp.} \\
		%
		\midrule
		%
		 & Q1.1 &How would you scale the level of realism of scenarios generated test cases in the \beamng simulator? & LS & \participantscount\\
	\multirow{5}{1cm}{\textbf{Evaluation based on \beamng }}	& Q1.2 &Justify  the level of realism of  scenarios  generated by test cases.  & OA & \participantscount \\
		& Q1.3 & How would you scale driving of AI \beamng  Simulator?   & LS & \participantscount \\
		& Q1.4 &  How would you scale overall experience with \beamng Simulator? & LS & \participantscount \\
		& Q1.5 & Justify overall experience with \beamng Simulator? & OA & \participantscount  \\
		%
		\midrule
		\multirow{9}{1cm}{\textbf{Evaluation based  on \carla}} & Q1.1 &How would you scale the level of realism of scenarios generated test cases in the \carla simulator? & LS & \participantscount \\
		& Q1.2 &Justify  the level of realism of  scenarios  generated by test cases.  & OA & \participantscount \\
		& Q1.3 & How would you scale driving of AI \carla Simulator?   & LS & \participantscount \\
		& Q1.4 &  How would you scale overall experience with \carla  Simulator? & LS & \participantscount \\
		& Q1.5 & Justify overall experience with \carla  Simulator? & OA & \participantscount  \\
		& Q1.6 & How do you compare safety with  Interaction and without interaction? & OA & \participantscount  \\
		%
		\midrule
		\multirow{2}{1cm}{\textbf{Feedback Section}} & Q3.1 & Did this experiment change the way you thought about the  Self-driving Cars safety? & MC & \participantscount  \\
		& Q3.1 & Please write in a few words on your experience and suggestions. & OA & \participantscount  \\
		\bottomrule
	\end{tabular}
%} %of resizebox 
	      \vspace{-2mm}
\end{table}


\subsection{Experimental procedure}\label{sec:experimental-procedure}

The overall experimental setup is illustrated in Figure \ref{fig:study-overview}. After the participants received a brief introduction on the study, the experiment started with both the \beamng and  \carla on-screen test cases (i.e., without VR), which includes three test cases for each simulator, with warmup tasks (no evaluation is required to familiarize oneself with the environment), consisting of the participants observing test cases without obstacles and test cases with obstacles. This preliminary activity was performed to allow participants to get familiar with the technologies that will be used in the study.
%After a \beamng simulator, we start with \carla test scenarios similar to \beamng.
Hence, for each test case generated (detailed in Section \ref {sec:test-generation}) the participants were asked to provide their view on their perception of safety and realism of test cases, with and without the VR, and for both driver and outside view (RQ1-3).
\seba{@christian, probably we have to be more clear on how participants could interact with the SDC in the next sentences, please improve it..}
In addition, experiments with additional test cases (detailed in Section \ref {sec:test-generation}) were conducted to investigate the extent to which the  perception of safety and realism of test cases of participants  vary when they can interact with the SDC (i.e., alter the behavior of the SDC). To interact with the SDCs the participants were provided with the ability to use a keyboard to slow down or accelerate the SDC’ behavior, depending on their level of perceived safety (e.g., decelerating when, in a certain moment, they felt the context of the test case was unsafe).

\subsubsection{Log \& Survey Data Collection and Analysis}. \seba{@Chrstian,   let’s improve as much as we can the following part..}.
For each test case in our dataset (detailed in Section \ref {sec:test-generation}), executed during each participant’s experiment, we collected all relevant data. Specifically, we save in JSON files the logs generated by the simulators \beamng and \carla after running the test cases. 
%These logs were stored locally on the experiment's computing infrastructure.
\seba{@chris, in the next sentence let’s  add references to examples of such files in the replication package.. }
Examples of \beamng and \carla logs can be found in our replication package %by following Listing ~\ref{lst:beamnglogs}. 
In such log files, we stored the time of logging, the coordinates of the vehicle's position, the sensor data (such as fuel, gear, and wheel speed, among others), an whether or not the SDC crossed the line (passing and failing test case according to the OOB metric) during the test case execution. 
 In addition, \framework classified the executed test cases as failing and passing and recorded the execution time (in the very same JSON log file). 
On \carla, the structure log has some additional information such as the details of weather conditions. 
%The example is found in the following listing: ~\ref{lst:carlalogs}. 
% and we asked them to justify their response. Similarly we asked to the participants, by using Likert scale, their level of perception of realism of executed test cases.
For both  \beamng and \carla simulators, we asked the participant to evaluate the test cases, considering the various questions reported in Table~\ref{tab:simulatorbasedsurvey}.
Hence, after each test case has been executed, we collected feedback information through surveys for each participant. Participants provided likert scale values to share their perceived level of safety and realism of each test case (see from Table \ref{table:option_assesssafety} an example of Likert scale range of values for safety). It is important to note that to further enhance our findings, we also analyze the quantitative and qualitative insights provided by the participants WITH or WITHOUT the VR headsets \todo{(the former is a case where the participant takes in the experiment primarily conducted on the screen of a computer while the latter focuses on the participant's experience when he/she is wearing a VR headset)} as well as when experiencing different driving views. 

%Each participant completed the experiment by producing two artefacts for each task: (i) \beamng and the \carla simulator generated logs. The logs include sensor data such as wind speed and car runtime coordinates; in the CARLA simulator, we also log information on dynamic weather conditions. 

\cb{Statistical analysis on Likert-scaled data is more challenging since many assumptions for "typical" methods do not hold, e.g., normality and continuity.}
\cb{Wilocoxon rank sum test is the same as Mann-Whitney U test but I guess the latter expression is more known, right?}
\todo{
A variety of visualizations/graphs, such as Stacked histograms and boxplots, are used to analyze and compare the safety and realism perception of participants.
In terms of statistical tests, we employed the \shapirowilk test to verify normality, the \mannwhitneyu test, and the \varghadelaney statistic to determine the effective size. 
For the research question RQ1-2, we mainly analyze responses that were recorded in the non-interactive sessions which had no participant interventions on the SDC behavior.
In RQ3 we wanted to investigate the effect that interactions with SDCs have on the participant’s perception of safety and realism of SDC test cases.
In order to analyze this difference in perception of safety/realism among the participants, we analyze both the close-ended questionnaire, i.e., participant survey scores, and open-ended questions including qualitative feedback. Histograms are used again to understand the spread of data across the two categories under consideration, i.e., test cases with interaction WITH the SDC and test cases WITHOUT interaction with the SDC. 
}
%To analyse the measures of central tendency across the two categories, box plots are used along with the statistical tests discussed in \RQ{3} to establish and prove the statistical significance of the difference between the two classes under question.

%We also log the users' interactions with the SDC into the logs in interaction scenarios; (ii) Level of safety evaluation with both close-ended and open-ended questions for statistical and qualitative analysis (RQ1-3).



\begin{table}[t] 
\scriptsize
\caption{Safety levels (Likert-scale intensity) }
\centering
\label{table:option_assesssafety}
\begin{tabularx}{\linewidth}{clX}\toprule
    \textbf{Likert scale} & \textbf{Safety options}     & \textbf{Example justification} \\
    \midrule
    5 & Very Safe                   & When passengers feel it is a dangerous threat \\   
    4 & Safe                        & When passengers feel it is a marginally less risk \\
    3 & Neutral                     & When passengers feel it is a normal situation   \\   
    2 & Unsafe                      & When passengers feel it is risk-free  \\   
    1 & Very Unsafe                 & When passengers feel extremely safe in the car \\ \bottomrule
\end{tabularx}
\end{table}

%\begin{figure}[h!]
%\centering
%\begin{minipage}{0.9\textwidth}
%\begin{lstlisting}[caption={Example \beamng logs },label={lst:beamnglogs},language=json,firstnumber=1]
%{
  %    "time": 0.03287863731384277,
   %   "position": [
     %   49.1695671081543,
      %  77.75309753417969,
      %  -27.797107696533203
      %],
      %”sensors": {
       % "_data": {
        %  "tcs": 0,
         % "fuel": 0.999969815320138,
         % "gear": 1,
         % "wheelspeed": 0.00015000228758618706,
          %….
        %}
      %}
    %}
%\end{lstlisting}
%\end{minipage}
%\end{figure}

%\begin{figure}[h!]
%\centering
%\begin{minipage}{0.7\textwidth}
%\begin{lstlisting}[caption={Example \carla logs },label={lst:carlalogs},language=json,firstnumber=1]
%{
  %  "simulation_data":[[
   %   "NO_ACTION",
    %  46.66442942619324,
   %   230.62664794921875,
  %    36.942161560058594,
 %     0.0016762923914939165
%    ],
%    [
%      "CHANGE_WEATHER",
%      46.66442942619324,
%      "Sun(alt: 4.73, azm: 191.29) Storm(clouds=48%, rain=8%, wind=40%)"
%    ],
%    [
%      "CAR_CROSSED_LINE",
%      46.66442942619324,
%      230.62664794921875,
%      36.942161560058594,
%      0.001712379395030439
%    ]]
%    }
%\end{lstlisting}
%\end{minipage}
%\end{figure}


==> sections/old/03-old-results.tex <==
\section{Results}\label{sec:results}
%To what extent does the OOB safety metric for simulation-based test cases of SDCs align with human safety assessments?
%- stacked-plot
%- box-plot:
%	- distribution of liker-scale (y-axis=user-perception-liker, x-axis=failing/passing-based-on-oob)
%	- group only failing and passing (regardless of VR)
%	- and statistically significant
%	- 
%- bar-plot
%- Only numerically / statisicall tests / stacked bars
%	- how vary the perception when using different simulator
%	- how vary the perception when using different views
%	- how vary the perception when using VR
%- boxplot:
%	- separate plot for failing and passing tests (grouped by complexity)
%	- separate plot for views (grouped by complexity)
%	- separate plot for VR/-No-VR (grouped by complexity)
%- stat. tests for all graphs!
%- Qualitative evaluation:
%	- insights supporting the quantitative results
%	- no taxonomy requires as for RQ2
%- multiple permutation test
%	- this is used to understand what factors impact most the perception of safety
%\cb{Plots are available on GitHub: \url{https://github.com/christianbirchler-org/ICSE-vr-study/tree/master/results}}
\cb{Consider to use barplots instead of boxplots due to discrete number scales.}

In this section, we present the results obtained from the survey conducted during the experiments with the participants.
Furthermore, we use the logs of \framework to observe the OOB metric if the test fails or passes (according to the OOB metric).
We report various combinations of potential factors that might influence the perception of safety by the users separately.



\subsection{\RQ{1}: Human-based assessment of SDC safety metrics}\label{sec:results-rq1}
%\pr{Main Result: Yes, the OOB metric matches the human perception of the safety of the test case. Then we talk about how different variables influence safety perception. For example, when individuals use VR, they feel more safe. Similarly, when individuals are inside or outside, they perceive bla bla.}

To answer \RQ{1}, we analyze the Likert scale values from different subgroups of the data.
For example, comparing the perceived safety of failing and passing tests, or the perceived safety from different view points with different complexity of the scenario.
In this way, we want to see what factors influences the results on the perceived safety described by the study participants.
For each subgropup we show boxplots and report statistical tests in Table~\ref{tab:rq1-statistical-test-results}.


%negligible 2|A12-0.5| < 0.147
%small 2|A12-0.5| < 0.33
%medium 2|A12-0.5| < 0.474
%large 2|A12-0.5| ≥ 0.474

%\begin{tblr}{
%  colspec={XXXX},
%  row{odd}={bg=lightgray},  
%  row{1}={bg=black,fg=white},
%}
\begin{table}[t]
    \centering
    \scriptsize
    \caption{Statistical test results for \RQ{1}}
    \begin{tblr}{
        colspec={|ccc|},
        cell{1}{1}={r=2}{c}, cell{1}{2}={r=2}{c}, cell{1}{3}={c},
        cell{3,8,13,18,23,28,33}{1}={c=3}{c},
        cell{4,9,14,19,24,29,34}{1}={r=2}{c},
        cell{1,4,5,7,9,10,12,14,15,17,19,20,22,24,25,27,29,30,32,34,35,37}{3}={bg=gray!50},
        cell{2,6,11,16,21,26,31,36}{3}={bg=blue!20},
        hline{8,13,18,23,28,33}={dashed},
        hline{17,18,22,23}={3}{1pt,red,solid},
        vline{3,4}={17,22}{1pt,red,solid},
        %cell{17,22}{3}={cmd=\fbox},
        }\toprule
        \textbf{Method} & \textbf{Test statistic} & \textbf{p-value} \\
         & & \textbf{Effect size $A_{12}$} \\ \midrule
         \underline{\emph{Failing vs. Passing (Figure~\ref{fig:rq1-1})}} && \\
%Failing vs Passing tests:
%	MannwhitneyuResult(statistic=40461.5, pvalue=6.177473859832768e-14)
%	ShapiroResult(statistic=0.8613325953483582, pvalue=3.690332713236406e-18)
%	ShapiroResult(statistic=0.9030535221099854, pvalue=4.4138401700949403e-13)
         \shapirowilk & $0.86$ & ** $3.69*10^{-18}$ \\
                                      & $0.90$  & ** $4.41*10^{-13}$ \\
        \varghadelaney &  & $0.34$ \\
        \mannwhitneyu & $40461.5$ & ** $6.2*10^{-14}$ \\
        
         \underline{\emph{Failing: No obstacles vs. with obstacles (Figure~\ref{fig:rq1-2})}} && \\
%	MannwhitneyuResult(statistic=26507.0, pvalue=3.524597233273335e-13)
%	ShapiroResult(statistic=0.9039194583892822, pvalue=4.710842382849023e-09)
%	ShapiroResult(statistic=0.7942952513694763, pvalue=2.1475480115294438e-16)
         \shapirowilk & $0.90$ & ** $4.71*10^{-9}$ \\
                                      & $0.79$  & ** $2.15*10^{-16}$ \\ 
        \varghadelaney &  & $0.71$ \\
        \mannwhitneyu & $26507.0$ & ** $3.52*10^{-16}$ \\ 
        
        \underline{\emph{Passing: No obstacles vs. with obstacles (Figure~\ref{fig:rq1-2})}} && \\
%Passing tests: no obstacles vs. with obstacles:
%	MannwhitneyuResult(statistic=12719.5, pvalue=0.058873853517748855)
%	ShapiroResult(statistic=0.8922946453094482, pvalue=5.075216913397185e-10)
%	ShapiroResult(statistic=0.9042337536811829, pvalue=1.5625798255314294e-07)
         \shapirowilk & $0.89$ & ** $5.08*10^{-10}$ \\
                                      & $0.90$  & ** $1.56*10^{-7}$ \\ 
        \varghadelaney &  & $0.56$ \\
        \mannwhitneyu & $12719.5$ & $0.06$ \\ 

%VR vs. No VR:
%	MannwhitneyuResult(statistic=36817.5, pvalue=0.16266202049710166)
%	ShapiroResult(statistic=0.8873403072357178, pvalue=1.7708058883897582e-16)
%	ShapiroResult(statistic=0.8820883631706238, pvalue=2.2639024335746605e-11)
         \underline{\emph{VR vs. No VR (without interactive scenarios) (Figure~\ref{fig:rq1-VR-vs-no-VR})}} && \\
         \shapirowilk & $0.89$ & ** $1.77*10^{-16}$ \\
                                      & $0.88$  & **$2.26*10^{-11}$ \\ 
        \varghadelaney &  & $0.47$ \\
        \mannwhitneyu & $36817.5$ & $0.16$ \\ 

%No VR outside view: no obstacles vs. with obstacles:
%	MannwhitneyuResult(statistic=6591.5, pvalue=6.736170655363249e-05)
%no_obstacles:	ShapiroResult(statistic=0.8910602331161499, pvalue=5.498355335475935e-07)
%with_obstacles	ShapiroResult(statistic=0.819430947303772, pvalue=1.0243921266805955e-09)
         \underline{\emph{No VR outside view: No obstacles vs. with obstacles (Figure~\ref{fig:rq1-3} and Figure~\ref{fig:rq1-VR-vs-no-VR-stacked-bar})}} && \\
         \shapirowilk & $0.89$ & ** $5.48*10^{-7}$ \\
                                      & $0.82$  & **$1.02*10^{-9}$ \\ 
        \varghadelaney &  & $0.66$ \\
        \mannwhitneyu & $6591.5$ & ** $6.74*10^{-5}$ \\ 
        
%VR outside view: no obstacles vs. with obstacles:
%	MannwhitneyuResult(statistic=6460.0, pvalue=0.00020746851722541794)
%no_obstacles:	ShapiroResult(statistic=0.8900755047798157, pvalue=4.968791813553253e-07)
%with_obstacles	ShapiroResult(statistic=0.8498150706291199, pvalue=1.1673856548100048e-08) 
         \underline{\emph{VR outside view: No obstacles vs. with obstacles (Figure~\ref{fig:rq1-3})}} && \\
         \shapirowilk & $0.89$ & ** $4.97*10^{-7}$ \\
                                      & $0.85$  & ** $1.17*10^{-8}$ \\ 
        \varghadelaney &  & $0.65$ \\
        \mannwhitneyu & $6460.0$ & ** $2.075*10^{-4}$ \\ 

%VR driver view: no obstacles vs. with obstacles:
%	MannwhitneyuResult(statistic=7082.5, pvalue=1.4546726793348463e-07)
%no_obstacles:	ShapiroResult(statistic=0.9040678143501282, pvalue=2.207385250585503e-06)
%with_obstacles	ShapiroResult(statistic=0.8295333981513977, pvalue=2.2298580759638753e-09)
         \underline{\emph{VR driver view: No obstacles vs. with obstacles (Figure~\ref{fig:rq1-3})}} && \\
         \shapirowilk & $0.90$ & ** $2.21*10^{-6}$ \\
                                      & $0.83$  & ** $2.23*10^{-9}$ \\ 
        \varghadelaney &  & $0.71$ \\
        \mannwhitneyu & $7082.5$ & ** $1.45*10^{-7}$ \\ \bottomrule
    \end{tblr}
    \label{tab:rq1-statistical-test-results}
\end{table}








%\subsubsection{Failing vs. Passing tests}
\subsubsection{Safety Perception of Failing vs. Passing test cases}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/results/RQ1/distribution-all-answers-boxplot.png}
    \caption{Perceived safety of failing and passing tests}
    \label{fig:rq1-1}
\end{figure}

Figure~\ref{fig:rq1-1} depicts the distribution of the perceiveid safety of test cases grouped by the test outcome (i.e., if the OOB metris is violated or not).
We observer a statistical significant difference (see Table~\ref{tab:rq1-statistical-test-results}) on how the participants perceive the safety of failing and passing test cases on a Likert scale.


\begin{finding}\label{find:rq1-1}
Overall, the passing tests (i.e., the OOB metric is not violated) have a higher perception of safety from the particpants than failing tests (OOB metric is violated).
\end{finding}

The above mentioned Finding~\ref{find:rq1-1} is coherent with several comments of the study participants (see Section~\ref{sec:comments-on-safety-perception}).
Those comments are associated with the \beamng simulator without VR and without obstacles.
We selected those comments since they focus soley on the lane-keeping ability of the car, i.e., they give qualitative insights on the OOB metric without influence of obstacles.
Most representative comments where the car violates the OOB metric (test is failing) are the following:
\begin{itemize}
    \item \textit{``As the car did not drive all the time on the street I felt unsafe. [...]'' (P3/B1/S1)}
    \item \textit{``When the car starts to go off the road when driving in a curve it feels pretty unsafe.'' (P31/B1/S1)}
    \item \textit{``Not Very Safe since the car sometimes drove a bit from the road.'' (P45/B1/S1)}
\end{itemize}

But also for passing tests where the OOB metric is not violated the participants gave comments like the following ones:
\begin{itemize}
    \item \textit{``The car was driving in lane and at a safe speed considering the road is empty.'' (P16/B1/S1)}
    \item \textit{``The car was following the path in a safety way and was not speeding up too much.'' (P25/B1/S1)}
\end{itemize}

All comments which support Finding~\ref{find:rq1-1} can be found in the Appendix~\ref{sec:comments-on-safety-perception}.



%\subsubsection{Failing and passing tests with different complexity}
\subsubsection{Safety Perception for Less/More complexity Test Cases}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/results/RQ1/failing-passing-tests-grouped-by-complexity-boxplot.png}
    \caption{Perceived safety of failing and passing tests grouped by scenario's complexity}
    \label{fig:rq1-2}
\end{figure}

Additionally to the first insights on failing and passing test cases, the participants also evaluated the test cases based on different complexity (i.e., if additional obstacles are included in the scene or not).
In Figure~\ref{fig:rq1-2} we observe a difference in the perceived safety when we group the tests into their complexity.
The difference is also statistical significant as reported in Table~\ref{tab:rq1-statistical-test-results}.
Concretely, failing test cases are perceived unsafer as the passing ones as aforementioned, however, when those failing test cases consists of additional obstacles then the perceived safety is even lower than the failing tests without obstacles.

In contrast to the case of passing tests, the perceived safety seems not to be significantly affected when the complexity of the scenario is higher (i.e., by additional obstacles).
Indeed, from Table~\ref{tab:rq1-statistical-test-results} (red cell) we see no statistical difference in the samples.
Those obsvervations leads us to the following finding:

\begin{finding}\label{find:failing-passing-complexity}
There is no statisical difference in the perception of safety when there are obstacles or no obstacles in the scenario when the OOB metric is not violated.
However, when the car goes out of bound the scenario is perceived unsafer if there are any obstacles ($p=3.52*10^{-16}$).
\end{finding}

From the participants we have also received answers which support the Finding~\ref{find:failing-passing-complexity}.
In case of participants who felt unsafe when obstacles were in the scene we obtained the following representative answers:
\begin{itemize}
    \item \textit{``The car crashed toward an obstacle and even running over bumps was not so smooth as humans would do. Definitively more unsafe that the previous scenario.'' (P1/B1/S2)}
    \item \textit{``Ran off the road in a curve and hit obstacles without slowing down, which resulted in flat tires.'' (P24/B1/S2)}
\end{itemize}

Comments of participants who felt safe or neutral when obstacles were in the scene:
\begin{itemize}
    \item \textit{``It car was running smooth with obstacles, there was a moment when it was too close to one of the obstacle.'' (P16/B1/S2)}
    \item \textit{``The vehicle does well to avoid obstacles while maintaining the safe speed.'' (P18/B1/S2)}
    \item \textit{``The driver accelerated over all the obsticles and did not have a perfect finish.'' (P40/B1/S2)}
    \item \textit{``Car was driving well. Only at the end it went off the road, but there was no object it bumped into.'' (P45/B1/S2)}
\end{itemize}

All comments which support Finding~\ref{find:failing-passing-complexity} are reported in the Appendix~\ref{sec:comments-on-safety-perception}.




\subsubsection{Safety perception with usage of VR and without VR}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imgs/results/RQ1/VR-NoVR-stacked-bar.png}
    \caption{VR vs. no VR}
    \label{fig:rq1-VR-vs-no-VR-stacked-bar}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imgs/results/RQ1/VR-NoVR-boxplot.png}
    \caption{VR vs. no VR}
    \label{fig:rq1-VR-vs-no-VR}
\end{figure}


To find out if the use of VR actually impact the perception of safety of the particanpts, we grouped the data also into \textit{with VR} and \textit{without VR}.
As reported in Table~\ref{tab:rq1-statistical-test-results}, we do not observe a statistical significant difference betwen those two groups.
However, from Figure~\ref{fig:rq1-VR-vs-no-VR-stacked-bar}, we see that in the case of \textit{without VR}, we have more participants reporting \textit{very safe} and \textit{very unsafe} than in the case of \textit{with VR}.
This observation is also illustrated in Figure~\ref{fig:rq1-VR-vs-no-VR} as the inter-quatile range of \textit{with VR} is smaller than the one of \textit{without VR}.
This leads us to the following finding:

\begin{finding}\label{find:VR-vs-no-VR}
The use of VR changed marginally the perception of safety.
When using VR the participants tend to feel the scenarios slightly unsafer.
However, the difference of perception is not statistical significant by the \mannwhitneyu test ($p=0.16$).
\end{finding}

Certain comments of participants support Finding~\ref{find:VR-vs-no-VR} such as
\begin{inparaenum}[(i)]
    \item \textit{``The prespective doesnt change much with the vr'' (P22/B2/S1)}, who reported to feel \neutral, or
    \item \textit{``The same as without the VR glasses. The car was not able to keep the middle of the lane and was driving badly compared to a human.'' (P28/B2/S1)}, who felt \veryunsafe.
\end{inparaenum}





\subsubsection{Different views with different complexity}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/results/RQ1/different-views-grouped-by-complexity-boxplot.png}
    \caption{Different views grouped by scenario's complexity}
    \label{fig:rq1-3}
\end{figure*}

As depicted in Figure~\ref{fig:rq1-3}, we observe a drop of perceived safety of the test cases among all different view points.
For all views we have statisical significant differences as shown in Table~\ref{tab:rq1-statistical-test-results}.
With the stasticial evidence for differences, we come up with the following finding:

\begin{finding}\label{find:different-view-with-different-complexity}
In general, from all view points, the participants perceived the test cases unsafer when obstacles are included.
\end{finding}

By looking on the general comments of the participant, which they made during the experiment for each simulator, they also qualitatively support Finding~\ref{find:different-view-with-different-complexity}.
For instance, the following representive comments were made on the \beamng driving behavior:
\begin{itemize}
    \item \textit{``the car meet with accident when it was tested with obstacles.'' (P11/B)}
    \item \textit{``didnt stick to the proper path most of the time. and also in the scenario 2 the ai ran into cylinder.'' (P13/B)}
    \item \textit{``It did not look at safety lines, which is very dangerous if other traffic is involved. It also ran off the road multiple times, which can easily lead to a loss of control. Also, the car rashed into easily avoidable obstacles.'' (P24/B)}
    \item \textit{``At least the AI seemes to have an understanding about the general elements of the simulation like the road. However, it seems to struggle with bumps in the middle of the road and also seems to drive to fast in curvy situations.'' (P31/B)}
    \item \textit{``The first scenario was always somehow ok, but not perfect enough to say it can go to the market. The second scenario is really not good.'' (P37/B)}
\end{itemize}

In the case of \carla, we got the following representative comments on the driving behavior with regard on different complexity of the scenario:
\begin{itemize}
 % Justify driving of AI CARLA Simulator ? 
 \item \textit{``In general it could keep the lane but sometimes the car made too sharp turns and did not stop for some stop signs.'' (P2/C)}
 \item \textit{``It crashed a lot and took strange paths on the street.'' (P3/C)}
 \item \textit{``It felt safer than beamNG because the car managed to follow narrower lanes, avoid realistic traffic and obey traffic lights.'' (P4/C)}
 \item \textit{``Driving was bit slow. It seems that it was taking time to make decision. But the driving looked safe except when it crashed into the roundabout.'' (P7/C)}
 \item \textit{``the ai was on the path most of the time except for the accident cases where it didnt handle it properly.'' (P13/C)}
 \item \textit{``It is not perfect and crushes occur. Still, I liked that the car also stopped at red lights without any difficulties. It was also always driving inside the markings of the road.'' (P23/C)}
 \item \textit{``Generally the AI followed the traffic rules, some crashes still happened but the driving was generally pretty good.'' (P24/C)}
 \item \textit{``Except at the round-abouts, the car followed traffic rules, signals and speed limits. However, it kept crashing and losing control in the round-abouts.'' (P27/C)}
 \item \textit{``In most scenarios the AI did well. From what I have seen during the simulations it is not able to drive around roundabouts and does not stop at stop signs.'' (P31/C)}
 \item \textit{``Very slow, ignores stops but mostly very good lane keeping.'' (P34/C)}
 \item \textit{``very slow driving, unsmooth behaviour, always to close to roundabout and abrupt stopping in front  of obstacles.'' (P41/C)}
\end{itemize}

We see that the perception of safety drops when increasing the complexity (i.e., adding obstacles to the scenario). This observation is coherent among both simulators, \beamng and \carla, as the participants reported so during the experiment.

%\cb{
%\begin{itemize}
%    \item Without VR the failing tests are perceived least safe but the passing ones most safe!
%    \item The dirver view with VR has almost no influence on safety perception!
%\end{itemize}
%}








\subsection{\RQ{2}: Human-based assessment of SDC realism}\label{sec:results-rq2}
%\pr{Main Result: We analyzed the passing and failing test cases, and for passing ones, we found that individuals perceive them as realistic. In contrast, for the failing ones, individuals perceive them as unrealistic. These results could vary based on the usage of VR and the views. For instance, the failing test cases could be perceived as more realistic when using VR.}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{imgs/results/RQ2/distribution-all-answers.png}
%    \caption{\cb{Distinguish between failing and passing tests.}}
%    \label{fig:rq1-overall-liker-scale-distribution}
%\end{figure}

%\cb{
%\begin{itemize}
%    \item GDoc of taxonomy process: \url{https://docs.google.com/document/d/1ukDDriU6sNLePDGLDeuny1YTOATA9_DUlAYESGTxZRI/edit?usp=sharing}
%    \item Taxonomy:
%    \begin{itemize}
%        \item Card sorting approach by Donna Spencer:
%        \begin{itemize}
%            \item \url{https://www.ipcinfo.org/fileadmin/user_upload/drm_matrix/docs/CardSorting-for-printing.pdf}
%            \item \url{https://medium.com/design-ibm/card-sorting-a-powerful-simple-research-method-9d1566be9b62}
%        \end{itemize}
%        \item Multiple coders (e.g., Teodora, Pooja, Christian)
%        \item Alignment of 2 coders to identify a category of match
%    \end{itemize}
%\end{itemize}
%}


\begin{table}[t]
    \centering
    \scriptsize
    \caption{Factors impacting the realism of the \beamng simulator}
    \begin{tblr}{
            colspec={lXr},
            row{1}={cmd=\textbf},
        }
        \toprule
        Category & Description & Occ. \\
        \midrule
        Audio & Auditive feedback from the simulator (e.g., sound of the engine, traffic, etc.) & 1 (2.0\%) \\
        Environment/Design & Visual accuracy of the rendered environment and obstacles (e.g., cars) & 14 (28.0\%) \\
        Road  & The accuracy of the road shapes reflecting real road scenarios. & 9 (18.0\%) \\
        Expected behavior & Is the simulator replicating the behaviors as expected in the real world? & 10 (20.0\%) \\
        Obstacles & Obstacles in the scene increases the complexity/realism & 15 (30.0\%) \\
        Surface/Ground & The accuracy on how the driving surface is rendered and the car should behave on it. & 12 (24.0\%) \\
        View point & E.g., driving, outside, etc. & 9 (18.0\%) \\
        Behavior/Dynamics & The dynamimcs during driving over or crashing into obstacles but also the reaction of the car while steering & 11 (22.0\%) \\
        Other comments & E.g., comparison with video games & 9 (18.0\%) \\
        \bottomrule
    \end{tblr}
    \label{tab:taxonomy-beamng}
\end{table}


\begin{table}[t]
    \centering
    \scriptsize
    \caption{Factors impacting the realism of the \carla simulator}
    \begin{tblr}{
            colspec={lXr},
            row{1}={cmd=\textbf},
        }
        \toprule
        Category & Description & Occ. \\
        \midrule
        Driving style  & of main car, of surrounding vehicles & 13 (26.0\%) \\
        Environment & Looks/Feels (weather, day, night...), Landscape looks (e.g., city), Traffic Looks/Details (e.g., lanes, stop signs, etc.), environmental obstacles (e.g., bikers, pedestrians, etc. & 28 (56.0\%) \\
        Audio & Auditive feedback from the simulator (e.g., sound of the engine, traffic, etc.) & 4 (8.0\%) \\
        Interaction & The possibility to interact with the car (e.g., adjusting the velocity) & 2 (4.0\%) \\
        Technicality & Resolution, Latency high/Lag, Graphics (e.g., textures, lightning), Physics of simulation  & 11 (22.0\%) \\
        Other comments & E.g., comparison with video games & 11 (22.0\%) \\
        \bottomrule
    \end{tblr}
    \label{tab:taxonomy-carla}
\end{table}

For evaluating the realism of both simulators (\beamng and \carla) we read and interpreted the comments of the 50 participants to find common factors which impact the perceived realism of the simulators and eventually defined a taxonomies for each simulator and a general meta-taxonomy.

\subsubsection{Realism in \beamng and \carla}
After two authors applied \textit{card sorting} to the user comments on the perceived realism (each author handled one simulator),  they defined for \beamng and \carla separate taxonomies on impacting factors on the perceived realism.
A third author refined the taxonomies resulting in a taxonomy for \beamng as depicted in Table~\ref{tab:taxonomy-beamng} and a taxonomy for  \carla in Table~\ref{tab:taxonomy-carla}.
The simulators have distinct factors that influence the perception of realism but also mutual ones.
For instance, in both simulators, the \textit{audio} and \textit{environment} are impacting factors.
The participants reported that if the audio is present and accurate, then it will increase the level of realism.
\todo{Quote a participant to support the statement in the previous sentence.}
The same applies to the environment; the perception of realism is impacted by the design and visual representation of the simulated elements in the environment.
\todo{Quote a participant to support the statement in the previous sentence.}
Next to the mutual factors, however, there are distinct factors as well for both simulators due to the different nature of the simulators.




\begin{finding}
\beamng and \carla have different factors impacting the perceived realism by the participants.
Only partially both simulators have mutual influencal aspects on realism such as the \textit{audio} and \textit{environment}.
\end{finding}


\begin{table}[t]
    \centering
    \scriptsize
    \caption{Meta taxonomy on factors impacting the perceive realism of simulation environments}
    \begin{tblr}{
            colspec={lXr},
            row{1}={cmd=\textbf}
        }
        \toprule
        Category & Description & Occ. \\
        \midrule
        Photorealism & Weather conditions, Landscape looks, Car design, Design of static objects (e.g., buildings, trees, sidewalk, etc.), traffic elements & \tbd \\
        Behavioral dynamics & Behavior of: Ego car, other vehicles (e.g., cars, motorbikes, bicycle, pedestrians) & \tbd \\
        Track/Lane & Shape, Dimensions, Structure, Materia & \tbd \\
        Traffic elements & E.g., other vehicles, road signs, cross-walks, etc. & \tbd \\
        Placement & Obstacles, objects & \tbd \\
        Rule system & Traffic restrictions/laws & \tbd \\
        Sensing & Acoustic perception, visual perception & \tbd \\
        \bottomrule
    \end{tblr}
    \label{tab:meta-taxonomy}
\end{table}

\subsubsection{Meta-taxonomy on realism}
Despite of some distinct factors impacting the perception of realism in \beamng and \carla, we define a general meta-taxonomy, which applies for both simulators.
For the second iteration of the \textit{card sorting}, the same two authors build a meta-taxonomy, which generalizes the impacting factors on the perceived realism independently from a specific simulator.
A third author revises the categories resulting in a meta-taxonomy as shown in Table~\ref{tab:meta-taxonomy}.
\cb{@Pooja: Can you review the taxonomies and give suggestions?}


\begin{finding}
\todo{Finding regarding the meta-taxonomy.}
\end{finding}



\subsection{\RQ{3}: Impact of human interaction on the assessments of SDCs}\label{sec:results-rq3}
\pr{Main Result: In state-of-the-art, the approaches to evaluate the safety of the test cases do not consider humans in the loop. When you involve humans in the loop and allow them to interact with the car (real-world setting), the individuals can perceive safety differently. We conjecture that humans feel safer when they can interact (control) with the car when necessary. Our results confirm that the perception of safety increases when individuals interact with the car. 
Safety is not static: We envision that future studies should include humans in the loop (the ability of humans to interact or control the car) when assessing static safety metrics for the test cases. 
}

%\subsection{\RQ{4}: Unsafe road segments from human perspective}\label{sec:results-rq4}

